Deep Multi-Task Networks For Occluded Pedestrian Pose Estimation

Most of the existing works on pedestrian pose estimation do not consider estimating the pose of an occluded pedestrian, as the annotations of the occluded parts are not available in relevant automotive datasets. For example, CityPersons, a well-known dataset for pedestrian detection in automotive scenes does not provide pose annotations, whereas MS-COCO, a non-automotive dataset, contains human pose estimation. In this work, we propose a multi-task framework to extract pedestrian features through detection and instance segmentation tasks performed separately on these two distributions. Thereafter, an encoder learns pose specific features using an unsupervised instance-level domain adaptation method for the pedestrian instances from both distributions. The proposed framework has improved state-of-the-art performances of pose estimation, pedestrian detection, and instance segmentation.

==> include/acknowledgement.tex <==
\section*{Acknowledgement}
We would like to thank Valeo for encouraging advanced research.

==> include/related_work.tex <==
\section{Related Work}

Pedestrian detection has been an extensively studied area of research % \cite{zhou2018bi, 
\cite{lin2018graininess, chen2018person} in the field of computer vision. With the recent successful attempts of detecting occluded pedestrians \cite{ouyang2017jointly, zhou2017multi}, HPE of the same subject has gained significant attention. In scenes where the pedestrian is occluded by other objects, HPE becomes extremely challenging. A first attempt to solve the problem was reported in ClueNet \cite{kishore2019cluenet}. Person-to-person occlusion remained a difficult problem which was further studied in \cite{das2020end} and solved in an unsupervised manner.

